High-Dimensional Geometric Streaming in Polynomial Space

Many existing algorithms for streaming geometric data analysis have been plagued by exponential dependencies in the space complexity, which are undesirable for processing high-dimensional data sets. In particular, once $d\geq\log n$, there are no known non-trivial streaming algorithms for problems such as maintaining convex hulls and L\"owner-John ellipsoids of $n$ points, despite a long line of work in streaming computational geometry since [AHV04]. We simultaneously improve these results to $\mathrm{poly}(d,\log n)$ bits of space by trading off with a $\mathrm{poly}(d,\log n)$ factor distortion. We achieve these results in a unified manner, by designing the first streaming algorithm for maintaining a coreset for $\ell_\infty$ subspace embeddings with $\mathrm{poly}(d,\log n)$ space and $\mathrm{poly}(d,\log n)$ distortion. Our algorithm also gives similar guarantees in the \emph{online coreset} model. Along the way, we sharpen results for online numerical linear algebra by replacing a log condition number dependence with a $\log n$ dependence, answering a question of [BDM+20]. Our techniques provide a novel connection between leverage scores, a fundamental object in numerical linear algebra, and computational geometry. For $\ell_p$ subspace embeddings, we give nearly optimal trade-offs between space and distortion for one-pass streaming algorithms. For instance, we give a deterministic coreset using $O(d^2\log n)$ space and $O((d\log n)^{1/2-1/p})$ distortion for $p>2$, whereas previous deterministic algorithms incurred a $\mathrm{poly}(n)$ factor in the space or the distortion [CDW18]. Our techniques have implications in the offline setting, where we give optimal trade-offs between the space complexity and distortion of subspace sketch data structures. To do this, we give an elementary proof of a "change of density" theorem of [LT80] and make it algorithmic.

==> online-sensitivity.tex <==
\section{Online Sensitivities}

\begin{Lemma}[Uniform leverage scores imply uniform $\ell_p$ sensitivities]\label{lem:uniform-l2-to-lp}
    Let $\bfA\in\mathbb R^{n\times d}$ and $2 < p < \infty$. Let $i\in[n]$. If $\bftau_i(\bfA) \leq \frac{\gamma d}{n}$, then $\bfs_i^p(\bfA) \leq \frac{(\gamma d)^{p/2}}{n}$.
\end{Lemma}
\begin{proof}
Let $\bfU$ be an orthonormal basis for the column space of $\bfA$. For any unit vector, we have that
\[
    \abs*{\bfu_i^\top\bfx}^p \leq \norm*{\bfu_i}_2^p \leq \parens*{\frac{\gamma d}{n}}^{p/2}
\]
by using the Cauchy--Schwarz and that $\norm*{\bfu_i}_2^2$ is the $i$th leverage score, and
\[
    \norm*{\bfU\bfx}_p^p \geq \norm*{\bfU\bfx}_2^p \cdot n^{1 - p/2} = n^{1-p/2}
\]
by H\"older's inequality and using that $\bfU$ is orthonormal. Thus,
\[
    \frac{\abs*{\bfu_i^\top\bfx}^p}{\norm*{\bfU\bfx}_p^p} \leq \frac{(\gamma d)^{p/2}n^{-p/2}}{n^{1-p/2}} = \frac{(\gamma d)^{p/2}}{n}
\]
for any $\bfx$. By taking the supremum over all unit vectors $\bfx$, we conclude as desired.
\end{proof}

\begin{Lemma}
    Let $\bfA\in\mathbb R^{n\times d}$ and $2 < p < \infty$. Let $\kappa$ be the condition number of $\bfA$. Then,
    \[
        \sum_{i=1}^n \bfs_i^{p,\mathsf{OL}}(\bfA) = O(d\log n\log\kappa).
    \]
\end{Lemma}
\begin{proof}
With Lemma \ref{lem:uniform-l2-to-lp} in hand, the modification of the proof of Lemma 4.7 of \cite{BDMMUWZ2020} is straightforward. 
\end{proof}

==> online-subspace-sketch.tex <==
\section{Online Subspace Sketch}

In this section, we consider subspace sketch problem in the row arrival streaming setting. Throughout this section, we assume that $\bfA\in\mathbb R^{n\times d}$ has integer entries bounded by $\poly(n)$. 

\subsection{One Pass Streaming Subspace Sketch: \texorpdfstring{$\poly(d)$}{poly(d)} Distortion, \texorpdfstring{$\poly(d)$}{poly(d)} Space}

Our main result for this section is an algorithm for computing a $\poly(d)$-distortion subspace sketch data structure for $\bfA\in\mathbb R^{n\times d}$ using $\poly(d)$ space, with one pass over a row arrival stream. Here, our space distortion bound is a polynomial with degree independent of $p$. We first show the algorithm for $\ell_\infty$, and then show how to modify it to obtain our algorithm for $\ell_p$.

\subsubsection{Algorithm for \texorpdfstring{$\ell_\infty$}{l inf}}

We first present a basic version of our algorithm. We will cover optimizations and variations of our algorithm in Section \ref{sec:streaming-subspace-sketch-opt-var}. Our algorithm is deterministic and computes a subset $S$ such that
\[
    \frac1\kappa \norm*{\bfA\bfx}_\infty \leq \norm*{\bfA\vert_S\bfx}_\infty \leq \norm*{\bfA\bfx}_\infty
\]
for all $\bfx\in\mathbb R^d$, for some $\kappa = O(d\sqrt{\log n})$.

\begin{algorithm}
	\caption{Streaming $\ell_\infty$ Subspace Sketch}
	\textbf{input:} $\bfA\in\mathbb R^{n\times d}$. \\
	\textbf{output:} Coreset $S\subseteq[n]$.
	\begin{algorithmic}[1] % The number tells where the line numbering should start
        \State $S\gets \varnothing$
        \For{$i\in[n]$}
            \If{$\exists\bfx\in\mathbb R^n$ : $\angle*{\bfa_i,\bfx}^2 \geq \norm*{\bfA\vert_S\bfx}_2^2$}\label{line:sensitivity-add-point}
                \State $S \gets S\cup\{i\}$
            \EndIf
        \EndFor
        \State \Return $S$
	\end{algorithmic}\label{alg:subspace-sketch-stream-l-inf}
\end{algorithm}

We show the following guarantee for Algorithm \ref{alg:subspace-sketch-stream-l-inf}:

\begin{Theorem}\label{thm:subspace-sketch-stream-l-inf}
    Let $\bfA\in\mathbb R^{n\times d}$ and let $S$ be the output of Algorithm \ref{alg:subspace-sketch-stream-l-inf}. Then:
    \begin{itemize}
        \item $\abs*{S} \leq O(d^2\log n)$
        \item $\frac1\kappa \norm*{\bfA\bfx}_\infty \leq \norm*{\bfA\vert_S\bfx}_\infty \leq \norm*{\bfA\bfx}_\infty$ for all $\bfx\in\mathbb R^d$, for $\kappa = O(d\sqrt{\log n})$. 
    \end{itemize}
    In particular, by storing the rows of $S$, we obtain an algorithm for the streaming $\ell_\infty$ subspace sketch problem using $O(d^3\log n)$ bits of space.
\end{Theorem}

To prove Theorem \ref{thm:subspace-sketch-stream-l-inf}, we need the following definitions and lemmas concerning the so-called \emph{online leverage scores} \cite{CMP2020,BDMMUWZ2020}, which are an ``online'' variant of the usual statistical leverage scores.

\begin{Definition}[Definition 2.1 of \cite{BDMMUWZ2020}, Theorem 2.2 of \cite{CMP2020}]
    Let $\bfA\in\mathbb R^{n\times d}$. Then, for each $i\in[n]$, the $i$th online leverage score is defined as
    \[
        \bftau_i^{\mathsf{OL}}(\bfA) \coloneqq \begin{cases}
            \min\{\bfa_i^\top(\bfA_{i-1}^\top\bfA_{i-1})^- \bfa_i,1\} & \bfa_i\in\rowspan(\bfA_{i-1}) \\
            1 & \text{otherwise}
        \end{cases}
    \]
    where $\bfA_{j}\in\mathbb R^{j\times d}$ denotes the submatrix of $\bfA$ formed by the first $j$ rows. 
\end{Definition}

Just as the sum of leverage scores is bounded by $d$ (Lemma \ref{lem:lewis-weights-sum-to-d}), the sum of online leverage scores is known to have a small sum, although not as small as their offline counterparts.

\begin{Lemma}[Lemma 2.2 of \cite{BDMMUWZ2020}, Theorem 2.2 of \cite{CMP2020}]\label{lem:online-leverage-score-bound}
    Let $\bfA\in\mathbb R^{n\times d}$ and let $\kappa = \kappa(\bfA)$ be the condition number of $\bfA$. Then,
    \[
        \sum_{i=1}^n \bftau_i^{\mathsf{OL}}(\bfA) = O(d\log\kappa).
    \]
\end{Lemma}

We require the following standard lemma relating online leverage scores and sensitivities:

\begin{Lemma}\label{lem:generalized-sensitivity}
    Let $\bfA\in\mathbb R^{n\times d}$ and $\bfa\in\rowspan(\bfA)$. Then,
    \[
        \sup_{\bfx\in\rowspan(\bfA)\setminus\{0\}} \frac{\angle*{\bfa,\bfx}^2}{\norm*{\bfA\bfx}_2^2} = \bfa^\top(\bfA^\top\bfA)^-\bfa.
    \]
\end{Lemma}
\begin{proof}
    Let $\bfA = \bfU\bfSigma\bfV^\top$ be the truncated SVD of $\bfA$. Then, $\bfa = \bfV\bfb$ for some $\bfb\in\mathbb R^{\rank(\bfA)}$. For any $\bfx\in\rowspan(\bfA)\setminus\{0\}$, let $\bfy = \bfSigma\bfV^\top\bfx$. Then,
    \begin{align*}
        \frac{\angle*{\bfa,\bfx}^2}{\norm*{\bfA\bfx}_2^2} &= \frac{\angle*{\bfV\bfSigma\bfSigma^{-1}\bfb,\bfx}^2}{\norm*{\bfU\bfy}_2^2} && \text{$\bfa = \bfV\bfb$} \\
        &= \frac{\angle*{\bfSigma^{-1}\bfb,\bfSigma\bfV^\top\bfx}^2}{\norm*{\bfy}_2^2} && \text{$\bfU$ has orthonormal columns} \\
        &= \angle*{\bfSigma^{-1}\bfb,\bfy/\norm*{\bfy}}^2 && \text{$\bfy = \bfSigma\bfV^\top\bfx$} \\
    \end{align*}
    The supremum over all $\bfx$ is equal to
    \[
        \norm*{\bfSigma^{-1}\bfb}_2^2 = \bfb^\top\bfSigma^{-2}\bfb
    \]
    by the Cauchy--Schwarz inequality and its tightness. This is equal to
    \[
        \bfa^\top(\bfA^\top\bfA)^-\bfa = \bfb^\top \bfV^\top (\bfV\bfSigma^2\bfV^\top)^- \bfV\bfb = \bfb^\top \bfSigma^{-2}\bfb.
    \]
    as claimed.
\end{proof}

Using the above, we prove Theorem \ref{thm:subspace-sketch-stream-l-inf}:

\begin{proof}[Proof of Theorem \ref{thm:subspace-sketch-stream-l-inf}]
We first bound $\abs*{S}$. Note that for every $i\in S$,
\[
    \bftau_i^{\mathsf{OL}}(\bfA\vert_S) = \Omega(1)
\]
since if $\bfa_i\in\rowspan((\bfA\vert_S)_{i-1})$, then by line \ref{line:sensitivity-add-point} and Lemma \ref{lem:generalized-sensitivity},
\[
    \bftau_i^{\mathsf{OL}}(\bfA\vert_S) = \sup_{\bfx\in\rowspan((\bfA\vert_S)_{i-1})\setminus\{0\}} \frac{\angle*{\bfa_i,\bfx}^2}{\norm*{(\bfA\vert_S)_{i-1}\bfx}_2^2} \geq 1
\]
while if $\bfa_i\notin\rowspan((\bfA\vert_S)_{i-1})$, then $\bftau_i^{\mathsf{OL}}(\bfA\vert_S) = 1$. However, the $\bftau_i^{\mathsf{OL}}(\bfA\vert_S)$ sum to $O(d\log \kappa(\bfA\vert_S))$ by Lemma \ref{lem:online-leverage-score-bound}, so it follows that $\abs*{S} \leq O(d\log \kappa(\bfA\vert_S))$. It is known that an $n\times d$ matrix with integer entries bounded by $\poly(n)$ has maximum singular value at most $\poly(n)$ and minimum singular value at least $1/\poly(n)^{O(d)}$ (see, e.g., Lemma 4.1 of \cite{CW2009}), so $\log \kappa(\bfA\vert_S) = O(d\log n)$, which gives a bound of
\begin{equation}\label{eq:l-inf-coreset-size-bound}
    \abs*{S}\leq O(d^2\log n)
\end{equation}

Next, we bound the distortion $\kappa$. Note that $\norm*{\bfA\vert_S\bfx}_\infty \leq \norm*{\bfA\bfx}_\infty$ is trivial, so it suffices to show the lower bound. Let $\bfx\in\mathbb R^d$ and let $i_*\in[n]$ satisfy $\norm*{\bfA\bfx}_\infty = \abs*{\angle*{\bfa_{i_*},\bfx}}$, i.e., the row that witnesses the max. If $i_*\in S$, then we already have that
\[
    \norm*{\bfA\vert_S\bfx}_\infty \geq \norm*{\bfA\bfx}_\infty
\]
so assume that $i_*\notin S$. Then,
\begin{align*}
    \norm*{\bfA\bfx}_\infty^2 &= \angle*{\bfa_{i_*},\bfx}^2 \\
    &\leq \norm*{\bfA\vert_S\bfx}_2^2 && \text{Line \ref{line:sensitivity-add-point}} \\
    &\leq \abs*{S}\cdot \norm*{\bfA\vert_S\bfx}_\infty^2 \\
    &\leq O(d^2\log n)\norm*{\bfA\vert_S\bfx}_\infty^2 && \text{Equation \eqref{eq:l-inf-coreset-size-bound}}
\end{align*}
which yields the claimed bound on $\kappa$.
\end{proof}

\subsubsection{Algorithm for \texorpdfstring{$\ell_p$}{lp}}

Given the $\ell_\infty$ subspace sketch algorithm, our result for $\ell_p$ for finite $p$ follows by embedding $\ell_p$ into $\ell_\infty$ via exponential random variables \cite{And2017, WZ2013}.

\begin{Definition}
    The exponential distribution is defined by its probability density function $f:[0,\infty)\to[0,1]$ via $f(x) = \exp(-x)$. If $X$ is distributed as an exponential, we write $X\sim\Exp$.
\end{Definition}

We use the following fact about exponential random variables:

\begin{Lemma}[Max stability, Property 1 of \cite{WZ2013}]\label{lem:max-stability}
    Let $E_1, \dots, E_n$ be i.i.d.\ and exponentially distributed. Let $\alpha_i > 0$ for $i\in[n]$. Then,
    \[
        \max\braces*{\frac{\alpha_1}{E_1}, \dots, \frac{\alpha_n}{E_n}} \sim \frac{\sum_{i=1}^n \alpha_i}{E}
    \]
    where $E$ is exponentially distributed.
\end{Lemma}

We then consider the following algorithm:

\begin{algorithm}
	\caption{Streaming $\ell_p$ Subspace Sketch}
	\textbf{input:} $\bfA\in\mathbb R^{n\times d}$, $0<p<\infty$. \\
	\textbf{output:} Coreset $S\subseteq[n]$, weights $\bfw_i$ for each $i\in S$.
	\begin{algorithmic}[1] % The number tells where the line numbering should start
        \State $S\gets \varnothing$
        \For{$i\in[n]$}
            \State $\bfw_i \gets E_i^{-1/p}$ with $E_i\sim \Exp$, $\bfW = \diag(\bfw)$\label{line:draw-exp}
            \If{$\exists\bfx\in\mathbb R^n$ : $\angle*{\bfw_i\bfa_i,\bfx}^2 \geq \norm*{\bfW\vert_S\bfA\vert_S\bfx}_2^2$}
                \State $S \gets S\cup\{i\}$
            \EndIf
        \EndFor
        \State \Return $S$, and $\bfw_i$ for each $i\in S$
	\end{algorithmic}\label{alg:subspace-sketch-stream-lp}
\end{algorithm}

Note that Algorithm \ref{alg:subspace-sketch-stream-lp} just corresponds to running Algorithm \ref{alg:subspace-sketch-stream-l-inf} with $\bfW\bfA$ instead of $\bfA$ for $\bfW$ as defined in line \ref{line:draw-exp}.

\begin{Theorem}\label{thm:streaming-subspace-sketch-lp-for-each}
    Let $\bfA\in\mathbb R^{n\times d}$ and let $S$ and $\bfw$ be the output of Algorithm \ref{alg:subspace-sketch-stream-lp}. Then:
    \begin{itemize}
        \item $\abs*{S} \leq O(d^2\log n)$
        \item for each $\bfx\in\mathbb R^d$,
        \[
            \Pr\braces*{\frac1{\kappa\log^{1/p}\frac1\delta} \norm*{\bfA\bfx}_p \leq \norm*{\bfW\vert_S\bfA\vert_S\bfx}_\infty\leq O\parens*{\frac1{\delta^{1/p}}}\norm*{\bfA\bfx}_p} \geq 1-\delta
        \]
        for $\kappa = O(d\sqrt{\log n})$. 
    \end{itemize}
    In particular, by storing the rows of $S$ scaled by the corresponding $\bfw_i$, we obtain an algorithm for the streaming $\ell_\infty$ subspace sketch problem using $O(d^3\log^2 n)$ bits of space.
\end{Theorem}
\begin{proof}
    Since Algorithm \ref{alg:subspace-sketch-stream-lp} just corresponds to running Algorithm \ref{alg:subspace-sketch-stream-l-inf} with $\bfW\bfA$ instead of $\bfA$ for $\bfW$ as defined in line \ref{line:draw-exp}, we immediately have that $\abs*{S} \leq O(d^2\log n)$ and that $\frac1\kappa \norm*{\bfW\bfA\bfx}_\infty \leq \norm*{\bfW\vert_S\bfA\vert_S\bfx}_\infty \leq \norm*{\bfW\bfA\bfx}_\infty$ for all $\bfx\in\mathbb R^d$. Note then that
    \[
        \norm*{\bfW\bfA\bfx}_\infty^p = \max_{i=1}^n \frac{\abs*{\angle*{\bfa_i,\bfx}}^p}{E_i} \sim \frac{\sum_{i=1}^n \abs*{\angle*{\bfa_i,\bfx}}^p}{E} = \frac{\norm*{\bfA\bfx}_p^p}{E}
    \]
    for some exponentially distributed random variable $E$, by Lemma \ref{lem:max-stability}. Since 
    \[
        \Pr\braces*{\frac\delta2 \leq E \leq \log\frac2\delta} \geq 1 - \delta,
    \]
    we conclude the statement of the theorem.
\end{proof}

Note that Theorem \ref{thm:streaming-subspace-sketch-lp-for-each} solves the streaming $\ell_p$ subspace sketch problem in the ``for each'' model. By repeating $O(d)$ times and taking the median, we obtain an algorithm in the ``for all'' model.

\begin{Corollary}\label{cor:streaming-subspace-sketch-lp-for-all}
    Let $\bfA\in\mathbb R^{n\times d}$ and $0<p<\infty$. There is a one pass row arrival streaming algorithm using $O(d^4\log^2 n)$ bits of space which outputs a data structure $Q_p:\mathbb R^d\to\mathbb R_{\geq0}$ such that
    \[
        \Pr\braces*{\forall\bfx\in\mathbb R^d,\frac1\kappa \norm*{\bfA\bfx}_p \leq Q_p(\bfx) \leq \norm*{\bfA\bfx}_p} \geq \frac23
    \]
    for $\kappa = O(d\sqrt{\log n})$. 
\end{Corollary}

Finally, we note that Theorem \ref{thm:streaming-subspace-sketch-lp-for-each} can be directly used to efficiently solve $\ell_p$ regression in a stream, due to the ``one-sided'' nature of the guarantee.

\begin{Corollary}[$\ell_p$ Regression in a Row Arrival Stream]\label{cor:streaming-lp-regression}
    Let $\bfA\in\mathbb R^{n\times d}$ and $\bfb\in\mathbb R^n$ and $0 < p \leq \infty$. Suppose the algorithm receives the $n\times(d+1)$ matrix $\bfA' \coloneqq [\bfA\ \bfb]$ in a row arrival stream. There is a one pass streaming algorithm such that:
    \begin{itemize}
        \item for $p = \infty$, the algorithm uses $O(d^3\log^2 n)$ bits of space and outputs $\hat\bfx\in\mathbb R^d$ such that $\norm*{\bfA\hat\bfx-\bfb}_\infty \leq O(d\sqrt{\log n}) \min_\bfx\norm*{\bfA\bfx-\bfb}_\infty$, deterministically
        \item for $0<p<\infty$, the algorithm uses $O(d^3\log^2 n)$ bits of space and outputs $\hat\bfx\in\mathbb R^d$ such that $\norm*{\bfA\hat\bfx-\bfb}_p\leq O(d^{1+1/p}\log^{1/2+1/p} n) \min_\bfx\norm*{\bfA\bfx-\bfb}_p$, with probability at least $2/3$
    \end{itemize}
\end{Corollary}
\begin{proof}
    The results for $p = \infty$ follow immediately from combining Theorem \ref{thm:subspace-sketch-stream-l-inf} with the sketch-and-solve paradigm (see, e.g., Theorem \ref{thm:lp-regression-large-distortion}). Note that $\ell_\infty$ regression can be solved efficiently in polynomial time using linear programming. See also \cite{EV2019} for recent work on fast $\ell_\infty$ regression solvers.

    For $0<p<\infty$, we use the fact that sketch-and-solve paradigm only requires a one-sided guarantee to solve linear regression (see, e.g., \cite{CW2015b}). More specifically, we show that
    \begin{equation}\label{eq:lower-bound-one-sided}
        \Pr\braces*{\forall\bfx\in\mathbb R^d, \norm*{\bfW\vert_S\bfA'\vert_S\bfx}_\infty \geq \frac1{O(d^{1+1/p}\log^{1/2+1/p} n)}\norm*{\bfA'\bfx}_p} \geq \frac{9}{10}
    \end{equation}
    and that for each $\bfx\in\mathbb R^d$,
    \begin{equation}\label{eq:upper-bound-one-sided}
        \Pr\braces*{\norm*{\bfW\vert_S\bfA'\vert_S\bfx}_\infty \leq O(1)\norm*{\bfA'\bfx}_p} \geq \frac{9}{10}.
    \end{equation}
    The second claim immediately follows from Theorem \ref{thm:streaming-subspace-sketch-lp-for-each} with $\delta = 1/10$. To prove the first claim, we use a standard net argument. 
    
    Let $\mathcal N \subseteq \colspan(\bfA')$ be a set of unit vectors of cardinality at most $\abs*{\mathcal N} \leq \exp(O(d\log n))$ such that for every $\ell_p$ unit vector $\bfy\in\colspan(\bfA')$, there exists $\bfy'\in\mathcal N$ such that $\norm*{\bfy-\bfy'}_p \leq 1/\poly(n)$. The existence of such a set is standard, see, e.g., Lemma 2.4 of \cite{BLM1989}. Then by choosing $\delta = 1/(10\abs*{\mathcal N})$ in Theorem \ref{thm:streaming-subspace-sketch-lp-for-each} and applying a union bound over $\mathcal N$, we have that
    \begin{equation}\label{eq:net-exp-vars}
        \Pr\braces*{\forall \bfy'\in\mathcal N,\norm*{\bfW\vert_S\bfy'\vert_S}_\infty \geq \frac1{O(d^{1+1/p}\log^{1/2+1/p} n)}\norm*{\bfy'}_p} \geq \frac{9}{10}
    \end{equation}
    Now let $\bfy\in\colspan(\bfA')$ be any unit vector. Then,
    \[
        \norm*{\bfW\vert_S\bfy\vert_S - \bfW\vert_S\bfy'\vert_S}_p \leq \norm*{\bfW}_\infty\norm*{\bfy - \bfy'}_p \leq O(n) \frac1{\poly(n)} = \frac1{\poly(n)}
    \]
    where we have used that $\norm*{\bfW}_\infty \leq O(n^{1/p})$ with constant probability. Thus, conditioned on the event of Equation \eqref{eq:net-exp-vars}, we have that
    \begin{align*}
        \norm*{\bfW\vert_S\bfy\vert_S}_p &\geq \norm*{\bfW\vert_S\bfy'\vert_S}_p - \norm*{\bfW\vert_S\bfy\vert_S - \bfW\vert_S\bfy'\vert_S}_p \\
        &\geq  \frac1{O(d^{1+1/p}\log^{1/2+1/p} n)} - \frac1{\poly(n)} = \frac1{O(d^{1+1/p}\log^{1/2+1/p} n)}
    \end{align*}
    which shows Equation \eqref{eq:lower-bound-one-sided}.

    With Equations \eqref{eq:lower-bound-one-sided} and \eqref{eq:upper-bound-one-sided} in hand, we can show that $\hat\bfx \coloneqq \arg\min_\bfx \norm*{\bfW\vert_S\bfA\vert_S\bfx - \bfW\vert_S\bfb\vert_S}_\infty$, which can be efficiently computed, satisfies
    \[
        \norm*{\bfA\hat\bfx-\bfb}_p \leq O(d^{1+1/p}\log^{1/2+1/p}n)\min_{\bfx\in\mathbb R^d}\norm*{\bfA\bfx-\bfb}_p
    \]
    exactly as in the proof of Theorem \ref{thm:lp-regression-large-distortion}.
\end{proof}

\subsubsection{Optimizations and Variations}\label{sec:streaming-subspace-sketch-opt-var}

\paragraph{Nearly Input Sparsity Time.}

Here, we show how to process the rows of $\bfA$ in batches to make Algorithm \ref{alg:subspace-sketch-stream-l-inf} run in input sparsity time. We first use the observation of \cite{CMP2020,BDMMUWZ2020} that batch processing of rows can only shrink the online leverage scores, since for a batch $B\subseteq[n]$ and a row $j\in B$,
\[
    \bftau_j^{\mathsf{OL}}(\bfA) = \sup_{\bfx}\frac{\angle*{\bfa_j,\bfx}^2}{\norm*{\bfA_{j-1}\bfx}_2^2} \geq \sup_{\bfx}\frac{\angle*{\bfa_j,\bfx}^2}{\norm*{\bfA_{B}\bfx}_2^2} = \bftau_j(\bfA_B).
\]
To determine the appropriate batch size, note that the size of the coreset $S$ is still at most $\abs*{S} \leq O(d^2\log n)$, so we only ever compute leverage scores of a matrix with $B + O(d^2\log n)$ rows. By Theorem \ref{thm:cohen-peng-fast-lewis-weights}, this requires time at most
\[
    \tilde O((\nnz(\bfA\vert_{B}) + d^3\log n) + d^\omega)
\]
Thus, if the batch size is $O(d^3\log n)$ rows, then the running time is at most $\tilde O(\nnz(\bfA))$.

\paragraph{Near Optimal Two Pass Algorithm.}

Observe that if every $O(d^2\log n)$ rows of $\bfA$ has condition number at most $\kappa = \poly(n)$, then Algorithm \ref{alg:subspace-sketch-stream-l-inf} for $\ell_\infty$ subspace sketch in fact finds a coreset of size $O(d\log\kappa) = O(d\log n)$ rather than $O(d^2\log n)$. This in turn improves the distortion of the subspace embedding to $O(\sqrt{d\log n})$, which is a space complexity and distortion bound which matches the offline guarantee achieved by L\"owner--John ellipsoids.

We show that we can in fact force this to occur, by taking an additional pass through the stream to condition the matrix, and then adding a small a perturbation to the matrix which conditions every small submatrix of $\bfA$ but only negligibly affects the $\ell_\infty$ norms of vectors in the subspace. 

\begin{Theorem}[Near Optimal Two Pass $\ell_\infty$ Subspace Sketch]\label{thm:two-pass-l-inf-subspace-sketch}
    There is an algorithm which makes two passes over a row arrival stream of $\bfA\in\mathbb R^{n\times d}$ and maintains a data structure $Q:\mathbb R^d \to \mathbb R$ such that
    \[
        \Pr\braces*{\forall\bfx\in\mathbb R^d,\norm*{\bfA\bfx}_\infty \leq Q_p(\bfx) \leq O(\sqrt{d\log n})\norm*{\bfA\bfx}_\infty} \geq \frac23.
    \]
    The algorithm uses $O(d^2\log^2 n)$ bits of space.
\end{Theorem}
\begin{proof}
    First note that by making an additional pass over the data, we can maintain $\bfM = \bfA^\top\bfA = \sum_{i=1}^n \bfa_i^\top\bfa_i$. Let $\bfM = \bfV\bfSigma^2\bfV^\top$ be an orthonormal eigendecomposition of $\bfM$. Note then that $\bfA\bfV\bfSigma^{-1}$ has orthonormal columns. In the second pass, we may then simulate a row arrival stream to $\bfU+\bfG$ for $\bfU = \bfA\bfV\bfSigma^{-1}$ and $\bfG\in\mathbb R^{n\times d}$ a matrix with entries distributed as i.i.d.\ Gaussians drawn from $\mathcal N(0,1/\poly(n))$, by accessing the rows as 
    \[
        (\bfu_i^\top+\bfg_i^\top) = \bfe_i^\top\bfU + \bfg_i^\top = \bfe_i^\top\bfA\bfV\bfSigma^{-1} + \bfg_i^\top = \bfa_i^\top\bfV\bfSigma^{-1} + \bfg_i^\top.
    \]
    With probability at least $1 - 1/\poly(n)$, all entries are at least $1/\poly(n)$ and at most $1/\poly(n)$ in absolute value, so we condition on this event. We may then round every coordinate of $\bfU+\bfG$ to $O(\log n)$ bits with relative error $(1\pm1/\poly(n))$ on every coordinate to obtain $\bfB$. 
    
    We now use a theorem from the study of smoothed analyses of condition numbers \cite{DST2011, TV2007, TV2010, BC2010}. By Theorem 1.1 of \cite{BC2010}, the condition number of any fixed $m\times d$ matrix $\bfC$ for $m \geq 2d$, perturbed by a i.i.d.\ Gaussians with variance $\sigma^2$, satisfies the following concentration inequality for $z$ sufficiently large:
    \[
        \Pr_{\bfC'\sim\mathcal N(\bfC,\sigma^2\bfI_{m\times d})}\braces*{\kappa(\bfC') \geq 2e\cdot z} \leq 4\bracks*{\parens*{6 + \sqrt{2\log(2z)} + \frac1{\sigma\sqrt{m}}}\frac1z}^{m-d+1} \leq \parens*{\frac{O(\sqrt{\log z})}{\sigma\sqrt{m}z}}^{m/2}.
    \]
    Note that there are at most $n^{m}$ submatrices formed by taking $m$ rows of $\bfB$. Then by choosing $z$ to be large enough in $\poly(n)$ (which is large enough to apply the above theorem of \cite{BC2010}) and taking a union bound, we find that all $m\times d$ submatrices of $\bfB$ have condition number at most $\poly(n)$, for all $2d \leq m \leq O(d^2\log n)$.  
    
    We will then run Algorithm \ref{alg:subspace-sketch-stream-l-inf} on the matrix $\bfB$. Then by the above discussion, the condition number of the coreset $S$ discovered by the algorithm is at most $\poly(n)$, so $S$ has size at most $O(d\log n)$ and the distortion is at most $O(\sqrt{d\log n})$.

    We now show how to answer queries. As usual, we may assume that $\bfx$ is in the row space of $\bfA$, since otherwise we may project onto it since we have stored $\bfA^\top\bfA$. Now for a query $\bfx$, let $\bfy = \bfSigma\bfV^\top\bfx$, so that $\bfA\bfx = \bfU\bfy$. Note that $\bfU$ is orthonormal, so for any unit vector $\bfx$, $\norm*{\bfU\bfy}_2^2 = \norm*{\bfy}_2^2$ and $\norm*{\bfU\bfy}_\infty^2 \geq \norm*{\bfy}_2^2/n$. On the other hand, $\norm*{\bfG\bfy}_\infty^2 \leq \norm*{\bfG\bfy}_2^2 \leq \norm*{\bfy}_2^2 / \poly(n)$ so by the triangle inequality, $\norm*{(\bfU+\bfG)\bfy}_\infty^2 = \Theta(\norm*{\bfU\bfy}_\infty^2)$. In turn, $\norm*{\bfB\bfy}_\infty^2 = \Theta(\norm*{\bfA\bfx}_\infty^2)$. Finally, by applying Theorem \ref{thm:subspace-sketch-stream-l-inf} on $\bfB$, we conclude that
    \[
        \norm*{\bfB\vert_S\bfy}_\infty \leq \Theta(1)\norm*{\bfA\bfx}_\infty \leq O(\sqrt{d\log n})\norm*{\bfB\vert_S\bfy}_\infty
    \]
    as desired.
\end{proof}

We similarly get an improvement for $\ell_p$ subspace sketch, although this is not optimal since one can get even better distortions and space in the offline setting for finite $p$.

\begin{Corollary}[Two Pass $\ell_p$ Subspace Sketch]\label{cor:two-pass-lp-subspace-sketch}
    Let $0<p<\infty$. There is an algorithm which makes two passes over a row arrival stream of $\bfA\in\mathbb R^{n\times d}$ and maintains a data structure $Q_p:\mathbb R^d \to \mathbb R$ such that
    \[
        \Pr\braces*{\forall\bfx\in\mathbb R^d,\norm*{\bfA\bfx}_p \leq Q_p(\bfx) \leq O(\sqrt{d\log n})\norm*{\bfA\bfx}_p} \geq \frac23.
    \]
    The algorithm uses $O(d^3\log^2 n)$ bits of space.
\end{Corollary}

\subsection{One Pass Streaming Subspace Sketch: \texorpdfstring{$(1+\eps)$}{(1+eps)} Distortion, \texorpdfstring{$d^{p/2+1}$}{d**(p/2+1)} Space}

We show the simple result of obtaining $(1+\eps)$ distortion in one pass via the merge and reduce framework (see, e.g., \cite{CDW2018,BDMMUWZ2020}).

\begin{Theorem}\label{thm:1+eps-merge-reduce-subspace-sketch}
    Let $\bfA\in\mathbb R^{n\times d}$, $0 < p < \infty$, and $\eps>0$. Then, there is a one pass streaming algorithm which uses $O(d^{2\lor(p/2+1)}\poly(\log n,\eps^{-1}))$ space and outputs a data structure $Q_p$ such that
    \[
        \Pr\braces*{\forall\bfx\in\mathbb R^d, \norm*{\bfA\bfx}_p \leq Q_p(\bfx) \leq (1+\eps)\norm*{\bfA\bfx}_p} \geq \frac23
    \]
\end{Theorem}
\begin{proof}
    We partition the $n$ rows of $\bfA$ into blocks of $B \coloneqq O(d^{1\lor (p/2)}\poly(\log n,\eps^{-1}))$ rows, and then merge them in a binary tree-like fashion, with depth $O(\log n)$. To merge two submatrices $\bfA_1$ and $\bfA_2$ each with $B$ rows, we apply Theorem \ref{thm:lewis-weight-subspace-embedding} with accuracy parameter set to $\eps/\log n$ and failure rate parameter set to $1/\poly(n)$ on the $2B\times d$ matrix $\bfB \coloneqq [\bfA_1^\top\ \bfA_2^\top]^\top$ to get back a $B\times d$ matrix $\bfB'$ such that
    \[
        \Pr\braces*{\forall\bfx\in\mathbb R^d, \norm*{\bfB\bfx}_p \leq \norm*{\bfB'\bfx}_p \leq \parens*{1+\frac{\eps}{\log n}}\norm*{\bfB\bfx}_p} \geq 1 - \frac1{\poly(n)}
    \]
    By a union bound over all $O(n)$ merge operations required to combine all $O(n)$ blocks, the above guarantee holds every time we merge two blocks. Furthermore, because the depth of the binary tree is at most $\floor{\log_2 n}$, the distortion is at most $1+\eps$.

    Finally, to argue the space bound, we inductively argue that the above merging scheme can be implemented by storing at most $O(\log n)$ blocks of rows at a time. Assume first that $n$ is a power of $2$. Then, for $n = 2$, we clearly store at most $\log_2 n + 1 = 2$ blocks at once. Now to merge $n$ blocks, we use at most $\log_2(n/2) + 1 = \log_2 n$ at once to get a single block merging the first $n/2$ blocks. We can then do this again to obtain a single block merging the next $n/2$ blocks. This used at most $1 + \log_2 n$ blocks at once. Padding proves the result for general $n$. Then, storing $O(\log n)$ blocks of size $B\times d$ requires $O(Bd\log n)$ space, which is the claimed space complexity.
\end{proof}

\subsection{Near-Optimal Bounds for Restricted Instances}

In this section, we study a restricted variant of the $\ell_\infty$ subspace sketch problem, and give near optimal algorithms and lower bounds. 

\begin{Definition}[Restricted $\ell_\infty$ Subspace Sketch]\label{def:restricted-subspace-sketch}
We define the restricted $\ell_\infty$ subspace sketch problem as follows. Let $\bfA\in\mathbb R^{n\times d}$ be a matrix with row norms all $\Theta(1)$. Then, we must design a data structure $Q$ that receives a row arrival stream of $\bfA$ and answers queries $\bfx\in\mathbb R^d$ at the end of the stream. Furthermore, we must output
\[
    Q(\bfx) \leq \kappa\norm*{\bfA\bfx}_\infty
\]
for all $\bfx\in\mathbb R^d$, while we must output
\[
    Q(\bfx) \geq \norm*{\bfA\bfx}_\infty
\]
when $\bfx$ is an input point, i.e., $\bfx$ is one of the rows $\bfa_i$ of $\bfA$.
\end{Definition}

We show that the lower bound instance of \cite{LWW2021} is captured by this restriction, and show an algorithm that matches the lower bound up to logarithmic factors.

\subsubsection{Lower Bound}

We will use the following lemma from coding theory, which has previously been used several times in streaming and communication lower bounds for linear algebraic problems \cite{LWW2021, MMWY2021}. 
\begin{Lemma}[\cite{PTB2013}]\label{lem:coding-random-points}
For any $p\geq 1$ and $d = 2^k - 1$ for some integer $k$, there exists a set $S\subseteq\{-1,1\}^d$ and a constant $C_p$ depending only on $p$ which satisfy
\begin{itemize}
    \item $\abs*{S} = d^p$
    \item For any $s,t\in S$ such that $s\neq t$, $\abs*{\angle*{s,t}} \leq C_p\sqrt d$
\end{itemize}
\end{Lemma}

We then have the following:

\begin{Theorem}\label{thm:restricted-subspace-sketch-lb}
    Let $n = d^q$ for some integer $q$. Suppose that a streaming algorithm $\mathcal A$ solves the restricted $\ell_\infty$ subspace sketch problem (Definition \ref{def:restricted-subspace-sketch}) with $\kappa = c\sqrt d$ for some sufficiently small constant $c>0$. Then, $\mathcal A$ must use $\Omega(n)$ bits of space.
\end{Theorem}
\begin{proof}
    We show the result by reduction from the \textsf{INDEX} problem (Theorem \ref{thm:index}). 

    Let $S\subseteq\{-1,1\}^d$ be the set of vectors given by Lemma \ref{lem:coding-random-points} with $n = d^q$. Suppose that Alice has a subset $A\subseteq[n]$. Then, Alice can feed the vectors of $S$ corresponding to her subset $A$, normalized to have norm $\Theta(1)$, and then pass the memory state of $\mathcal A$ to Bob. Now suppose that Bob has the index $b\in [n]$. Then, Bob queries the subspace sketch data structure the vector $\bfx_b\in S$ corresponding to the index $b$.
    
    If $b\in A$, then we have that $Q(\bfx_b) \geq \norm*{\bfA\bfx_b}_\infty = \norm*{\bfx_b}_2^2 = \Theta(1)$. On the other hand, if $b\notin A$, then we have that
    \[
        Q(\bfx_b) \leq \kappa \norm*{\bfA\bfx}_\infty \leq c\sqrt d \cdot \frac1{\Theta(\sqrt d)} = \Theta(c).
    \]
    Thus for $c$ sufficiently small, Bob can distinguish whether $b\in A$ or not and thus $\mathcal A$ must use at least $\Omega(n)$ bits of space.
\end{proof}


\begin{Remark}
By replacing our use of Lemma \ref{lem:coding-random-points} with $n$ random unit vectors in $d$ dimensions, we can instead get a collection of vectors with inner product $\Theta(\sqrt{(\log n)/d})$, which leads to an $\Omega(n)$ bit lower bound for distortions better than $O(\sqrt{d/\log n})$, even for $n$ larger than $\poly(d)$.
\end{Remark}

\subsubsection{Upper Bound}

In this section, we design an algorithm solving the restricted $\ell_\infty$ subspace sketch problem (Definition \ref{def:restricted-subspace-sketch}). Our algorithm is given in Algorithm \ref{alg:l-inf-input-query-unit}.

\begin{algorithm}
	\caption{Restricted $\ell_\infty$ Subspace Sketch}
	\textbf{input:} $\bfA\in\mathbb R^{n\times d}$ in a row arrival stream of $\Theta(1)$ norm rows. \\
	\textbf{output:} Coreset $S\subseteq[n]$.
	\begin{algorithmic}[1] % The number tells where the line numbering should start
        \State $S\gets\varnothing$
        \For{$i\in[n]$}
            \If{there is no $j\in S$ s.t. $\abs*{\angle*{\bfa_j/\norm*{\bfa_j}_2,
            \bfa_i/\norm*{\bfa_i}_2}} \geq 1/\sqrt{2d-1}$}\label{line:keep-row}
                \State $S\gets S \cup \{i\}$
            \EndIf
        \EndFor
	\end{algorithmic}\label{alg:l-inf-input-query-unit}
\end{algorithm}

Our analysis will use the well-known Welch bound from coding theory.

\begin{Theorem}[Inner Product Lower Bound \cite{Wel1974}]\label{thm:inner-product-lb}
    Let $\bfa_1, \bfa_2, \dots, \bfa_M \in\mathbb R^d$ be a set of $M$ unit vectors. Let $k\geq 1$ be an integer. Then,
    \[
        \max_{i\neq j}\abs*{\angle*{\bfa_i,\bfa_j}}^{2k} \geq \frac1{M-1}\bracks*{\frac{M}{\binom{d+k-1}{k}} - 1}
    \]
\end{Theorem}

Using Theorem \ref{thm:inner-product-lb}, we show the following.

\begin{Theorem}\label{thm:restricted-subspace-sketch-alg}
    Let $\bfA\in\mathbb R^{n\times d}$ be a matrix with rows with norm $\Theta(1)$. Then, Algorithm \ref{alg:l-inf-input-query-unit} outputs a coreset $S\subseteq[n]$ such that
    \[
        C\sqrt d\norm*{\bfA_S\bfa_i}_\infty \geq \norm*{\bfA\bfa_i}_\infty
    \]
    for all $i\in[n]$, for some $C>0$ a sufficiently large constant. Furthermore, Algorithm \ref{alg:l-inf-input-query-unit} uses $O(d^2\log n)$ bits of space.
\end{Theorem}

Before proving Theorem \ref{thm:restricted-subspace-sketch-alg}, note that the result implies that Algorithm \ref{alg:l-inf-input-query-unit} solves the restricted $\ell_\infty$ subspace sketch problem, since trivially, we have that
\[
    C\sqrt d\norm*{\bfA_S\bfx}_\infty \leq C\sqrt d\norm*{\bfA\bfx}_\infty
\]
for all $\bfx\in\mathbb R^d$. 

\begin{proof}[Proof of Theorem \ref{thm:restricted-subspace-sketch-alg}]
First note that by assuming that $\bfa_i$ are unit vectors, we only lose $\Theta(1)$ factors in the distortion parameter $\kappa$, so we make this assumption without loss of generality. 

Note that the correctness guarantee is trivial from the construction of the algorithm, since every input point that doesn't satisfy line \ref{line:keep-row} is kept by the coreset. It suffices to argue the space complexity of the algorithm. 

We will argue that the algorithm keeps at most $O(d)$ points in $S$. If we apply Theorem \ref{thm:inner-product-lb} with $k = 1$ and $M = 2d$, we get that for any set of $M = 2d$ unit vectors $\bfa_1, \bfa_2, \dots, \bfa_M \in\mathbb R^d$,
\[
    \max_{i\neq j}\abs*{\angle*{\bfa_i,\bfa_j}}^{2} \geq \frac1{2d-1}\bracks*{\frac{2d}{d} - 1} = \frac1{2d-1}
\]
and thus the algorithm cannot keep more than $2d-1$ points. Storing these points only requires $O(d^2\log n)$ bits of space.
\end{proof}
